A Variational Approach to Bayesian Phylogenetic Inference

Bayesian phylogenetic inference is currently done via Markov chain Monte Carlo (MCMC) with simple proposal mechanisms. This hinders exploration efficiency and often requires long runs to deliver accurate posterior estimates. In this paper, we present an alternative approach: a variational framework for Bayesian phylogenetic analysis. We propose combining subsplit Bayesian networks, an expressive graphical model for tree topology distributions, and a structured amortization of the branch lengths over tree topologies for a suitable variational family of distributions. We train the variational approximation via stochastic gradient ascent and adopt gradient estimators for continuous and discrete variational parameters separately to deal with the composite latent space of phylogenetic models. We show that our variational approach provides competitive performance to MCMC, while requiring much fewer (though more costly) iterations due to a more efficient exploration mechanism enabled by variational inference. Experiments on a benchmark of challenging real data Bayesian phylogenetic inference problems demonstrate the effectiveness and efficiency of our methods.

==> figs/bn-reversed.tex <==
\input{rooted_tree}
\tikz[scale=0.75]{
  \begin{scope}[xscale=0.52, yscale=0.52, transform shape]
  \node[obs](S1){\scalebox{1.8}{$S_1$}};
  \node[obs, right=of S1, xshift=0.75cm, yshift=1.8cm](S2){\scalebox{1.8}{$S_2$}};
  \node[obs, right=of S1, xshift=0.75cm, yshift=-1.8cm](S3){\scalebox{1.8}{$S_3$}};
  \node[obs, right=of S2, xshift=0.75cm, yshift=1.8cm](S4){\scalebox{1.8}{$S_4$}};
  \node[obs, right=of S2, xshift=0.75cm, yshift=-0.6cm](S5){\scalebox{1.8}{$S_5$}};
  \node[obs, right=of S3, xshift=0.75cm, yshift=0.6cm](S6){\scalebox{1.8}{$S_6$}};
  \node[obs, right=of S3, xshift=0.75cm, yshift=-1.8cm](S7){\scalebox{1.8}{$S_7$}};
  \node[obs, right=of S4, xshift=0.75cm, yshift=1.8cm](S8){\scalebox{1.8}{$\cdots$}};
  \node[obs, right=of S4, xshift=0.75cm, yshift=0.25cm](S9){\scalebox{1.8}{$\cdots$}};
  \node[obs, right=of S5, xshift=0.75cm, yshift=1.05cm](S10){\scalebox{1.8}{$\cdots$}};
  \node[obs, right=of S5, xshift=0.75cm, yshift=-0.45cm](S11){\scalebox{1.8}{$\cdots$}};
  \node[obs, right=of S6, xshift=0.75cm, yshift=0.45cm](S12){\scalebox{1.8}{$\cdots$}};
  \node[obs, right=of S6, xshift=0.75cm, yshift=-1.05cm](S13){\scalebox{1.8}{$\cdots$}};
  \node[obs, right=of S7, xshift=0.75cm, yshift=-0.25cm](S14){\scalebox{1.8}{$\cdots$}};
  \node[obs, right=of S7, xshift=0.75cm, yshift=-1.8cm](S15){\scalebox{1.8}{$\cdots$}};
  \edge{S1}{S2, S3} ;
  \edge{S2}{S4, S5} ;
  \edge{S3}{S6, S7} ;
  \edge{S4}{S8, S9};
  \edge{S5}{S10, S11};
  \edge{S6}{S12, S13};
  \edge{S7}{S14, S15};
  \path (S1) edge [->, >={triangle 45}, bend right=10, dashed]  (S5);
  \path (S1) edge [->, >={triangle 45}, bend right=-30, dashed]  (S4);
  \path (S1) edge [->, >={triangle 45}, bend right=-10, dashed]  (S6);
  \path (S1) edge [->, >={triangle 45}, bend right=30, dashed]  (S7);
  \path (S2) edge [->, >={triangle 45}, bend right=5, dashed]  (S9);
  \path (S2) edge [->, >={triangle 45}, bend right=-30, dashed]  (S8);
  \path (S2) edge [->, >={triangle 45}, bend right=-5, dashed]  (S10);
  \path (S2) edge [->, >={triangle 45}, bend right=20, dashed]  (S11);
  \path (S3) edge [->, >={triangle 45}, bend right=-20, dashed]  (S12);
  \path (S3) edge [->, >={triangle 45}, bend right=5, dashed]  (S13);
  \path (S3) edge [->, >={triangle 45}, bend right=-5, dashed]  (S14);
  \path (S3) edge [->, >={triangle 45}, bend right=20, dashed]  (S15);
  \end{scope}
  
%  \begin{scope}[xscale=0.52, yscale=0.52, transform shape, xshift=16cm, yshift=-1cm]
%  \node[obs, yshift=4cm] (T1SP1) {\scalebox{1.2}{$\dfrac{ABC}D$}};
%
%  \node[obs, right=of T1SP1, xshift=0.5cm, yshift=1.1cm](T1SP2){\scalebox{1.2}{$\dfrac{A}{BC}$}};
%  \node[obs, right=of T1SP1, xshift=0.7cm, yshift=-1.1cm, fill=gray!10, draw=gray, densely dashed](T1SP3){\scalebox{1.8}{$D$}};
%  \node[obs, right=of T1SP2, xshift=0.5cm, yshift=1.1cm, fill=gray!10, draw=gray, densely dashed](T1SP4) {\scalebox{1.8}{$A$}};
%  \node[obs, right=of T1SP2, xshift=0.4cm, yshift=-0.35cm](T1SP5) {\scalebox{1.2}{$\dfrac{B}C$}};
%  \node[obs, right=of T1SP3, xshift=.75cm, yshift=0.35cm, fill=gray!10, draw=gray, densely dashed] (T1SP6) {\scalebox{1.8}{$D$}};
%  \node[obs, right=of T1SP3, xshift=.75cm, yshift=-1.1cm, fill=gray!10, draw=gray, densely dashed] (T1SP7) {\scalebox{1.8}{$D$}};
%    
%  \edge{T1SP1}{T1SP2} 
%  \annotatededge[densely dashed, gray!50]{pos=0.3, below=1pt}{1.0}{T1SP1}{T1SP3};
%  \annotatededge[densely dashed, gray!50]{pos=0.3, above=2pt}{1.0}{T1SP2}{T1SP4};
%  \edge{T1SP2}{T1SP5};
%  \annotatededge[densely dashed, gray!50]{pos=0.3, above=2pt}{1.0}{T1SP3}{T1SP6};
%  \annotatededge[densely dashed, gray!50]{pos=0.3, below=1pt}{1.0}{T1SP3}{T1SP7};
%  
%  
%  \node[obs, yshift=-2.5cm] (T2SP1) {\scalebox{1.2}{$\dfrac{AB}{CD}$}};
%  \node[obs, right=of T2SP1, xshift=0.5cm, yshift=1.1cm] (T2SP2) {\scalebox{1.2}{$\dfrac{A}{B}$}};
%  \node[obs, right=of T2SP1, xshift=0.5cm, yshift=-1.1cm] (T2SP3) {\scalebox{1.2}{$\dfrac{C}{D}$}};
%  \node[obs, right=of T2SP2, xshift=0.75cm, yshift=1.1cm, fill=gray!10, draw=gray, densely dashed] (T2SP4) {\scalebox{1.8}{$A$}};
%  \node[obs, right=of T2SP2, xshift=0.75cm, yshift=-0.4cm, fill=gray!10, draw=gray, densely dashed] (T2SP5) {\scalebox{1.8}{$B$}};
%  \node[obs, right=of T2SP3, xshift=0.75cm, yshift=0.4cm, fill=gray!10, draw=gray, densely dashed] (T2SP6) {\scalebox{1.8}{$C$}};
%  \node[obs, right=of T2SP3, xshift=0.75cm, yshift=-1.1cm, fill=gray!10, draw=gray, densely dashed] (T2SP7) {\scalebox{1.8}{$D$}}; 
%  
%  \edge{T2SP1}{T2SP2, T2SP3};
%  \annotatededge[densely dashed, gray!50]{pos=0.3, above=2pt}{1.0}{T2SP2}{T2SP4};
%  \annotatededge[densely dashed, gray!50]{pos=0.3, below=1pt}{1.0}{T2SP2}{T2SP5};
%  \annotatededge[densely dashed, gray!50]{pos=0.3, above=2pt}{1.0}{T2SP3}{T2SP6};
%  \annotatededge[densely dashed, gray!50]{pos=0.3, below=1pt}{1.0}{T2SP3}{T2SP7};
%  
%  \end{scope}   

%  \begin{scope}[xscale=0.52, yscale=0.52, transform shape, yshift=-1cm, xshift=30cm]
%  \node[yshift=2.2cm] (T1S1) {};
%  \node[left=2.5cm of T1S1, xshift=-2cm, yshift=1.6cm] (T1Arrow) {};
%  \draw[<->, >=stealth, thick] (T1Arrow) -- +(1.5,0);
%  \node[right=of T1S1, xshift=0.5cm, yshift=3.2cm](T1S2) {};
%  \node[leaf, right=of T1S1, xshift=3.48cm] (T1D) {\scalebox{1.4}{$D$}};
%  \node[leaf, right=of T1S2, xshift=1.8cm, yshift=0.75cm] (T1A) {\scalebox{1.4}{$A$}};
%  \node[right=of T1S2, xshift=0.5cm, yshift=-1.2cm] (T1S3) {};
%  \node[leaf, right=of T1S3, yshift=0.6cm] (T1B) {\scalebox{1.4}{$B$}};
%  \node[leaf, right=of T1S3, yshift=-0.6cm] (T1C) {\scalebox{1.4}{$C$}};
%  \csquaredge[thick]{T1S1}{T1S2}
%  \csquaredgeleaf[thick] {T1S1}{T1D};
%   \csquaredgeleaf[thick] {T1S2}{T1A};
%  \csquaredge[thick]{T1S2}{T1S3};
%  \csquaredgeleaf[thick]{T1S3}{T1B, T1C};
%  
%  
%  \node[yshift=-2.5cm] (T2S1) {};
%  \node[left=2.5cm of T2S1, xshift=-2cm] (T2Arrow) {};
%  \draw[<->, >=stealth, thick] (T2Arrow) -- +(1.5, 0);
%  \node[right=of T2S1, xshift=0.75cm, yshift=1.25cm] (T2S2) {};
%  \node[right=of T2S1, xshift=0.75cm, yshift=-1.25cm] (T2S3) {};
%  \node[leaf, right=of T2S2, xshift=1.45cm, yshift=0.75cm] (T2A) {\scalebox{1.4}{$A$}};
%  \node[leaf, right=of T2S2, xshift=1.45cm, yshift=-0.6cm] (T2B) {\scalebox{1.4}{$B$}};
%  \node[leaf, right=of T2S3, xshift=1.45cm, yshift=0.6cm] (T2C) {\scalebox{1.4}{$C$}};
%  \node[leaf, right=of T2S3, xshift=1.45cm, yshift=-0.75cm] (T2D) {\scalebox{1.4}{$D$}};
%  \csquaredge[thick]{T2S1}{T2S2, T2S3};
%  \csquaredgeleaf[thick]{T2S2}{T2A, T2B};
%  \csquaredgeleaf[thick]{T2S3}{T2C, T2D};
%  \end{scope}
  
%
%
%  \node[xshift=1.4cm, yshift=-2.5cm]  {$(a)$};
%  \node[xshift=9.49cm, yshift=-2.5cm] {$(b)$};
}

==> figs/bn.tex <==
\input{rooted_tree}
\tikz[scale=0.68]{
  \begin{scope}[xscale=0.52, yscale=0.52]
  \node [] (SA) at (0,2.25) {\scalebox{0.8}{Species A:}};
  \node [] (SB) at (0,0.75) {\scalebox{0.8}{Species B:}};
  \node [] (SC) at (0,-0.75) {\scalebox{0.8}{Species C:}};
  \node [] (SD) at (0,-2.25) {\scalebox{0.8}{Species D:}};
  \foreach \x/\c/\s in {2.7/red/A, 3.4/blue/T, 4.1/purple/G, 4.8/red/A, 5.5/red/A, 6.2/green/C}
  	\node at (\x, 2.3) {\tt{\textcolor{\c}{\s}}};
  \node at (7.3, 2.25) {\scalebox{0.7}{$\cdots$}};
  \foreach \x/\c/\s in {2.7/red/A, 3.4/blue/T, 4.1/purple/G, 4.8/green/C, 5.5/red/A, 6.2/green/C}
  	\node at (\x, 0.85) {\tt{\textcolor{\c}{\s}}};
  \node at (7.3, 0.75) {\scalebox{0.7}{$\cdots$}};
  \foreach \x/\c/\s in {2.7/red/A, 3.4/blue/T, 4.1/purple/G, 4.8/green/C, 5.5/red/A, 6.2/blue/T}
  	\node at (\x, -0.68) {\tt{\textcolor{\c}{\s}}};
  \node at (7.3, -0.75) {\scalebox{0.7}{$\cdots$}};
  \foreach \x/\c/\s in {2.7/red/A, 3.4/blue/T, 4.1/purple/G, 4.8/green/C, 5.5/red/A, 6.2/blue/T}
  	\node at (\x, -2.18) {\tt{\textcolor{\c}{\s}}};
  \node at (7.3, -2.25) {\scalebox{0.7}{$\cdots$}};
  \end{scope} 
  
  \begin{scope}[xscale=0.52, yscale=0.52, transform shape, xshift=11cm, yshift=-0.6cm]
  \node[yshift=2.2cm] (T1S1) {};
  \node[right=of T1S1, xshift=0.5cm, yshift=3.0cm](T1S2) {};
  \node[leaf, right=of T1S1, xshift=3.48cm] (T1D) {\scalebox{1.4}{$D$}};
  \node[leaf, right=of T1S2, xshift=1.8cm, yshift=0.95cm] (T1A) {\scalebox{1.4}{$A$}};
  \node[right=of T1S2, xshift=0.5cm, yshift=-1.0cm] (T1S3) {};
  \node[leaf, right=of T1S3, yshift=0.6cm] (T1B) {\scalebox{1.4}{$B$}};
  \node[leaf, right=of T1S3, yshift=-0.6cm] (T1C) {\scalebox{1.4}{$C$}};
  \csquaredge[thick]{T1S1}{T1S2}
  \csquaredgeleaf[thick] {T1S1}{T1D};
   \csquaredgeleaf[thick] {T1S2}{T1A};
  \csquaredge[thick]{T1S2}{T1S3};
  \csquaredgeleaf[thick]{T1S3}{T1B, T1C};
  
  
  \node[yshift=-2.5cm] (T2S1) {};
  \node[right=of T2S1, xshift=0.75cm, yshift=1.25cm] (T2S2) {};
  \node[right=of T2S1, xshift=0.75cm, yshift=-1.25cm] (T2S3) {};
  \node[leaf, right=of T2S2, xshift=1.45cm, yshift=0.75cm] (T2A) {\scalebox{1.4}{$A$}};
  \node[leaf, right=of T2S2, xshift=1.45cm, yshift=-0.6cm] (T2B) {\scalebox{1.4}{$B$}};
  \node[leaf, right=of T2S3, xshift=1.45cm, yshift=0.6cm] (T2C) {\scalebox{1.4}{$C$}};
  \node[leaf, right=of T2S3, xshift=1.45cm, yshift=-0.75cm] (T2D) {\scalebox{1.4}{$D$}};
  \csquaredge[thick]{T2S1}{T2S2, T2S3};
  \csquaredgeleaf[thick]{T2S2}{T2A, T2B};
  \csquaredgeleaf[thick]{T2S3}{T2C, T2D};
  \end{scope}
  
  \begin{scope}[xscale=0.52, yscale=0.52, transform shape, xshift=23cm, yshift=-0.6cm]
  \node[obs, yshift=4cm] (T1SP1) {\scalebox{1.4}{$\dfrac{ABC}D$}};
  \node[left=2cm of T1SP1, xshift=-1cm] (T1Arrow) {};
  \draw[<->, >=stealth] (T1Arrow) -- +(1.5,0);
  \node[obs, right=of T1SP1, xshift=0.5cm, yshift=1.1cm](T1SP2){\scalebox{1.4}{$\dfrac{A}{BC}$}};
  \node[obs, right=of T1SP1, xshift=0.8cm, yshift=-1.1cm, fill=gray!10, draw=gray, densely dashed](T1SP3){\scalebox{2.0}{$D$}};
  \node[obs, right=of T1SP2, xshift=0.5cm, yshift=1.1cm, fill=gray!10, draw=gray, densely dashed](T1SP4) {\scalebox{2.0}{$A$}};
  \node[obs, right=of T1SP2, xshift=0.4cm, yshift=-0.35cm](T1SP5) {\scalebox{1.4}{$\dfrac{B}C$}};
  \node[obs, right=of T1SP3, xshift=.75cm, yshift=0.35cm, fill=gray!10, draw=gray, densely dashed] (T1SP6) {\scalebox{2.0}{$D$}};
  \node[obs, right=of T1SP3, xshift=.75cm, yshift=-1.1cm, fill=gray!10, draw=gray, densely dashed] (T1SP7) {\scalebox{2.0}{$D$}};
    
  \edge{T1SP1}{T1SP2} 
  \annotatededge[densely dashed, gray!50]{pos=0.3, below=1pt}{}{T1SP1}{T1SP3};
  \annotatededge[densely dashed, gray!50]{pos=0.3, above=2pt}{}{T1SP2}{T1SP4};
  \edge{T1SP2}{T1SP5};
  \annotatededge[densely dashed, gray!50]{pos=0.3, above=2pt}{}{T1SP3}{T1SP6};
  \annotatededge[densely dashed, gray!50]{pos=0.3, below=1pt}{}{T1SP3}{T1SP7};
  
  
  \node[obs, yshift=-2.5cm] (T2SP1) {\scalebox{1.4}{$\dfrac{AB}{CD}$}};
  \node[left=2cm of T2SP1, xshift=-1cm] (T2Arrow) {};
  \draw[<->, >=stealth] (T2Arrow) -- +(1.5, 0);
  \node[obs, right=of T2SP1, xshift=0.65cm, yshift=1.1cm] (T2SP2) {\scalebox{1.4}{$\dfrac{A}{B}$}};
  \node[obs, right=of T2SP1, xshift=0.65cm, yshift=-1.1cm] (T2SP3) {\scalebox{1.4}{$\dfrac{C}{D}$}};
  \node[obs, right=of T2SP2, xshift=0.75cm, yshift=1.1cm, fill=gray!10, draw=gray, densely dashed] (T2SP4) {\scalebox{2.0}{$A$}};
  \node[obs, right=of T2SP2, xshift=0.75cm, yshift=-0.4cm, fill=gray!10, draw=gray, densely dashed] (T2SP5) {\scalebox{2.0}{$B$}};
  \node[obs, right=of T2SP3, xshift=0.75cm, yshift=0.4cm, fill=gray!10, draw=gray, densely dashed] (T2SP6) {\scalebox{2.0}{$C$}};
  \node[obs, right=of T2SP3, xshift=0.75cm, yshift=-1.1cm, fill=gray!10, draw=gray, densely dashed] (T2SP7) {\scalebox{2.0}{$D$}}; 
  
  \edge{T2SP1}{T2SP2, T2SP3};
  \annotatededge[densely dashed, gray!50]{pos=0.3, above=2pt}{}{T2SP2}{T2SP4};
  \annotatededge[densely dashed, gray!50]{pos=0.3, below=1pt}{}{T2SP2}{T2SP5};
  \annotatededge[densely dashed, gray!50]{pos=0.3, above=2pt}{}{T2SP3}{T2SP6};
  \annotatededge[densely dashed, gray!50]{pos=0.3, below=1pt}{}{T2SP3}{T2SP7};
  
  \node[right=of T1SP5, xshift=0.85cm, yshift=-0.7cm] (N1Arrowout) {};
  \path (N1Arrowout) edge[<-, >=stealth] node[pos=0.5, above=1pt, font=\LARGE, sloped]{assign} +(1.3,-0.75);
  \node[right=of T2SP6, xshift=0.85cm, yshift=0.7cm] (N2Arrowout) {};
  \path (N2Arrowout) edge[<-, >=stealth] node[pos=0.5, below=1pt, font=\LARGE, sloped]{assign}+(1.3,0.75);
  
  \end{scope}
  
  \begin{scope}[xscale=0.6, yscale=0.6, transform shape, xshift=30.5cm]
  \node[obs, xshift=4cm, yshift=3cm] (NS4) {\scalebox{1.8}{$S_4$}};
  \node[obs, xshift=4cm, yshift=1cm] (NS5) {\scalebox{1.8}{$S_5$}};
  \node[obs, xshift=4cm, yshift=-1cm] (NS6) {\scalebox{1.8}{$S_6$}};
  \node[obs, xshift=4cm, yshift=-3cm] (NS7) {\scalebox{1.8}{$S_7$}};
  
  \node[obs, left=of NS4, xshift=-0.5cm, yshift=-1.6cm] (NS2) {\scalebox{1.8}{$S_2$}};
  \node[obs, below=of NS2, yshift=-0.85cm] (NS3) {\scalebox{1.8}{$S_3$}};
  \node[obs, left=of NS2, xshift=-0.2cm, yshift=-1.4cm] (NS1) {\scalebox{1.8}{$S_1$}};
  
  \edge {NS2}{NS4, NS5};
  \edge {NS3}{NS6, NS7};
  \edge {NS1}{NS2, NS3};
  \end{scope}
  
%  \node[] at (1.25, -4) () {(a)};
%  \node[] at (7.5, -4) () {(b)};
%  \node[] at (13.5, -4) () {(c)};
%  \node[] at (19.25,-4) () {(d)};
}

==> rooted_tree.tex <==

% Clade node
\tikzstyle{clade} = [latent, rectangle, minimum size=18pt, node distance=2]

% Leaf node
\tikzstyle{leaf} = [font=\fontsize{15}{15}\selectfont, node distance=2]

% \squaredge  [options]  {inputs}  {outputs}
\newcommand{\squaredge}[3][] {
  % Connect all nodes #2 to all node #3.
  \foreach \x in {#2} {
    \foreach \y in {#3} {
      \draw[semithick, #1]  (\x) -- (\x |- \y) -- (\y);
    };
  };
}

% \csquaredge [options] {inputs} {outputs}
\newcommand{\csquaredge}[3][] {
  % Connect all nodes #2 to all node #3.
  \foreach \x in {#2} {
    \foreach \y in {#3} {
      \draw[semithick, #1]  (\x.center) -- (\x |- \y) -- (\y.center);
    };
  };
}

\newcommand{\undiredge}[5][] {
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#4} {
    \foreach \y in {#5} {
      \path (\x.center) edge[#1] node[pos=0.5, below, #2]{#3} (\y.center);
      };
    };
}

\newcommand{\undiredgeleaf}[5][] {
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#4} {
    \foreach \y in {#5} {
      \path (\x.center) edge[#1]node[pos=0.5, below, #2]{#3} (\y);
      };
    };
}


% \csquaredgeleaf [options] {inputs} {outputs}
\newcommand{\csquaredgeleaf}[3][] {
  % Connect all nodes #2 to all node #3.
  \foreach \x in {#2} {
    \foreach \y in {#3} {
      \draw[semithick, #1]  (\x.center) -- (\x |- \y) -- (\y);
    };
  };
}

% \annotatededge [options] [options] {edge value} {inputs} {outputs}
\newcommand{\annotatededge}[5][] {
 % Connect all nodes #2 to all node #3
 \foreach \x in {#4} {
   \foreach \y in {#5} {
     \path (\x) edge [->, >={triangle 45}, #1] node [pos=0.5, below, #2] {#3} (\y);
     };
   };
}
   
% \undirannotatededge [options][options] {edge value} {inputs} {outputs}
\newcommand{\undirannotatededge}[5][] {
 % Connect all nodes #2 to all nodes #3
 \foreach \x in {#4} {
   \foreach \y in {#5} {
     \path (\x) edge[#1] node [pos=0.5, below, #2] {#3} (\y);
   };
 };

}
      


